Off-Policy Evaluation Using Information Borrowing and Context-Based Switching

We consider the off-policy evaluation (OPE) problem in contextual bandits, where the goal is to estimate the value of a target policy using the data collected by a logging policy. Most popular approaches to the OPE are variants of the doubly robust (DR) estimator obtained by combining a direct method (DM) estimator and a correction term involving the inverse propensity score (IPS). Existing algorithms primarily focus on strategies to reduce the variance of the DR estimator arising from large IPS. We propose a new approach called the Doubly Robust with Information borrowing and Context-based switching (DR-IC) estimator that focuses on reducing both bias and variance. The DR-IC estimator replaces the standard DM estimator with a parametric reward model that borrows information from the 'closer' contexts through a correlation structure that depends on the IPS. The DR-IC estimator also adaptively interpolates between this modified DM estimator and a modified DR estimator based on a context-specific switching rule. We give provable guarantees on the performance of the DR-IC estimator. We also demonstrate the superior performance of the DR-IC estimator compared to the state-of-the-art OPE algorithms on a number of benchmark problems.

==> 05-Simulations.tex <==


\section{Experimental Setup}

In this section we outline the steps used for our experimental setup. For the choice of datasets, we follow Dudik (2011) to transform the classification datasets \texttt{glass}, \texttt{optdigits} and \texttt{yeast} into offline policy evaluation datasets. Specifically, the predicted label becomes the action taken, and the classification error becomes the observed loss $l$. Note that this is equivalent to observing a reward $r$, under the transformation $r=1-l$.

 \begin{figure*}[htbp]
% \vspace{-0.2cm}
	\centering
	\begin{minipage}{.47\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/glass_rmse_fixedrewards_drs_alpha1.png}
% 		\captionof{figure}{}
% 		\label{}
	\end{minipage}
	\begin{minipage}{.47\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/yeast_rmse_fixedreward_drs.png}
% 		\captionof{figure}{}
% 		\label{}
	\end{minipage}
 \caption{\it Glass (left) and Yeast (right) for four methods shown across 20 experiments for different sample sizes, $\alpha=1$. DR (red), Switch (magenta), corr switch (blue), oracle switch (black), oracle corr sw (green)}
 \label{fig5cs}
\end{figure*}

\begin{figure*}[htbp]
% \vspace{-0.2cm}
	\centering
	\begin{minipage}{.47\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/ecoli_fixed_rmse_drs_R.png}
% 		\captionof{figure}{}
% 		\label{}
	\end{minipage}
	\begin{minipage}{.47\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/ecoli_random_rmse_drs_R.png}% 		\captionof{figure}{}
% 		\label{}
	\end{minipage}
 \caption{\it Ecoli dataset with fixed (left) and random (right) reward model for five methods shown across 20 experiments for different sample sizes. DR (red), Switch (magenta), DR-IC(blue), oracle switch (black), oracle DR-IC (green)}
 \label{figecoli}
\end{figure*}
\begin{enumerate}
\item
We split the data into two parts- a training set, and a test set. We generate a context-dependent logging policy based on the training set, and use the generated logging policy to generate the actions. Towards this end, we generate actions uniformly, and develop a multinomial logistic model without intercept terms to train a policy. Once the policy is trained, we use the trained policy to generate the actions for the entire dataset.
\item
We use the training dataset to generate an evaluation policy through a multinomial logistic model, but using the true labels and losses for each combination of contexts in training set and possible actions. We use the evaluation policy to predict the actions in the testing set, and calculate the expected resultant loss, which forms the ground truth in subsequent steps.
\item
We use the training set to train the Direct methods, and use the testing set to evaluate the methods. We generate the actions for the testing set according to the trained logging policy $2000$ times to train the doubly robust methods, and obtain the bias and mse with respect to the ground truth.
\item
For our proposed approach, we optimize the bandwidth parameter over a grid using the predicted rmse with respect to the ground truth.
\end{enumerate}
FIXED REWARD RESULTS:
% \begin{figure*}[b]
%  \vspace{.3in}
%  \centerline{\fbox{\begin{tabular}{cc}
% \includegraphics[width=0.43\linewidth]{Figures/glass_rmse_fixedrewards_drs_alpha1.png} &
% \includegraphics[width=0.43\linewidth]{Figures/yeast_rmse_fixedreward_drs.png}\\
% %\includegraphics[width=0.49\linewidth]{glass_alpha1_bias_boxplot_n1070.png} &
% %\includegraphics[width=0.49\linewidth]{glass_alpha1_rmse_boxplot_n1070.png}\\
% \end{tabular}}}
%  \vspace{.3in}
%  \caption{\it Glass (left) and Yeast (right) for four methods shown across 20 experiments for different sample sizes, $\alpha=1$. DR (red), Switch (magenta), corr switch (blue), oracle switch (black), oracle corr sw (green)}
%  \label{fig5cs}
%  \end{figure*}
 






